An Effective Branch-and-Bound Algorithm with New Bounding Methods for the Maximum $s$-Bundle Problem

The Maximum s-Bundle Problem (MBP) addresses the task of identifying a maximum s-bundle in a given graph. A graph G=(V, E) is called an s-bundle if its vertex connectivity is at least |V|-s, where the vertex connectivity equals the minimum number of vertices whose deletion yields a disconnected or trivial graph. MBP is NP-hard and holds relevance in numerous realworld scenarios emphasizing the vertex connectivity. Exact algorithms for MBP mainly follow the branch-and-bound (BnB) framework, whose performance heavily depends on the quality of the upper bound on the cardinality of a maximum s-bundle and the initial lower bound with graph reduction. In this work, we introduce a novel Partition-based Upper Bound (PUB) that leverages the graph partitioning technique to achieve a tighter upper bound compared to existing ones. To increase the lower bound, we propose to do short random walks on a clique to generate larger initial solutions. Then, we propose a new BnB algorithm that uses the initial lower bound and PUB in preprocessing for graph reduction, and uses PUB in the BnB search process for branch pruning. Extensive experiments with diverse s values demonstrate the significant progress of our algorithm over state-of-the-art BnB MBP algorithms. Moreover, our initial lower bound can also be generalized to other relaxation clique problems.

==> body/05-Details.tex <==
The Maximum s-Bundle Problem (MBP) addresses the task of identifying a maximum s-bundle in a given graph. A graph G = (V, E) is called an s-bundle if its vertex connectivity is at least |V| - s, where the vertex connectivity equals the minimum number of vertices whose deletion yields a disconnected or trivial graph. MBP is NP-hard and holds relevance in numerous real-world scenarios emphasizing the vertex connectivity. Exact algorithms for MBP mainly follow the branch-and-bound (BnB) framework, whose performance heavily depends on the quality of the upper bound on the cardinality of a maximum s-bundle and the initial lower bound with graph reduction. In this work, we introduce a novel Partition-based Upper Bound (PUB) that leverages the graph partitioning technique to achieve a tighter upper bound compared to existing ones. To increase the lower bound, we propose to do short random walks on a clique to generate larger initial solutions. Then, we propose a new BnB algorithm that uses the initial lower bound and PUB in preprocessing for graph reduction, and uses PUB in the BnB search process for branch pruning. Extensive experiments with diverse s values demonstrate the significant progress of our algorithm over state-of-the-art BnB MBP algorithms. Moreover, our initial lower bound can also be generalized to other relaxation clique problems.

==> tabs/compare-intances.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[]
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l|rr|rrrrrrrr|rrrrrrrr}\toprule
\multirow{3}{*}{Instance} &
  \multicolumn{1}{c}{\multirow{3}{*}{$|V|$}} &
  \multicolumn{1}{c|}{\multirow{3}{*}{$|E|$}} &
  \multicolumn{8}{c|}{$s=2$} &
  \multicolumn{8}{c}{$s=8$} \\ \cline{4-19} 
 &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{4}{c|}{\name} &
  \multicolumn{2}{c|}{MSB} &
  \multicolumn{2}{c|}{RDS} &
  \multicolumn{4}{c|}{\name} &
  \multicolumn{2}{c|}{MSB} &
  \multicolumn{2}{c}{RDS} \\
 &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{$|V'|$} &
  \multicolumn{1}{c}{$|E'|$} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c|}{Time} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c|}{Time} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c|}{Time} &
  \multicolumn{1}{c}{$|V'|$} &
  \multicolumn{1}{c}{$|E'|$} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c|}{Time} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c|}{Time} &
  \multicolumn{1}{c}{Tree} &
  \multicolumn{1}{c}{Time} \\ \hline
bio-dmela &
  7393 &
  25569 &
  151 &
  621 &
  \textbf{0.522} &
  \multicolumn{1}{r|}{\textbf{0.217}} &
  149.8 &
  \multicolumn{1}{r|}{94.61} &
  8983 &
  1494 &
  2288 &
  15498 &
  \textbf{1695} &
  \multicolumn{1}{r|}{\textbf{119.5}} &
  1807 &
  \multicolumn{1}{r|}{338.5} &
  NA &
  NA \\
bio-pdb1HYS &
  36417 &
  36417 &
  189 &
  4341 &
  \textbf{0.322} &
  \multicolumn{1}{r|}{\textbf{0.750}} &
  8.889 &
  \multicolumn{1}{r|}{2.936} &
  NA &
  NA &
  60 &
  1632 &
  \textbf{10.76} &
  \multicolumn{1}{r|}{\textbf{2.699}} &
  498.4 &
  \multicolumn{1}{r|}{28.65} &
  NA &
  NA \\
ca-AstroPh &
  17903 &
  196972 &
  113 &
  3136 &
  \textbf{0.060} &
  \multicolumn{1}{r|}{\textbf{4.070}} &
  91.52 &
  \multicolumn{1}{r|}{1377} &
  NA &
  NA &
  267 &
  7269 &
  \textbf{1.093} &
  \multicolumn{1}{r|}{\textbf{8.628}} &
  476.9 &
  \multicolumn{1}{r|}{1862} &
  NA &
  NA \\
ca-dblp-2010 &
  226413 &
  716460 &
  455 &
  13491 &
  \textbf{0.574} &
  \multicolumn{1}{r|}{\textbf{272.9}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  844 &
  21716 &
  \textbf{2.327} &
  \multicolumn{1}{r|}{\textbf{327.6}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
ca-dblp-2012 &
  317080 &
  1049866 &
  216 &
  11592 &
  \textbf{0.106} &
  \multicolumn{1}{r|}{\textbf{448.6}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  216 &
  11592 &
  \textbf{0.160} &
  \multicolumn{1}{r|}{\textbf{396.0}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
c-fat200-1 &
  200 &
  1534 &
  90 &
  729 &
  \textbf{0.001} &
  \multicolumn{1}{r|}{\textbf{0.011}} &
  0.704 &
  \multicolumn{1}{r|}{0.019} &
  3.757 &
  0.031 &
  200 &
  1534 &
  \textbf{28.63} &
  \multicolumn{1}{r|}{\textbf{0.954}} &
  32.23 &
  \multicolumn{1}{r|}{0.976} &
  NA &
  NA \\
c-fat200-5 &
  200 &
  8473 &
  116 &
  4147 &
  \textbf{0.148} &
  \multicolumn{1}{r|}{0.147} &
  2.164 &
  \multicolumn{1}{r|}{\textbf{0.049}} &
  2.565 &
  0.083 &
  200 &
  8473 &
  \textbf{1720} &
  \multicolumn{1}{r|}{\textbf{75.78}} &
  1724 &
  \multicolumn{1}{r|}{81.74} &
  NA &
  NA \\
c-fat500-1 &
  500 &
  4459 &
  140 &
  1351 &
  \textbf{0.294} &
  \multicolumn{1}{r|}{\textbf{0.035}} &
  1.669 &
  \multicolumn{1}{r|}{0.117} &
  19.84 &
  0.301 &
  500 &
  4459 &
  \textbf{350.0} &
  \multicolumn{1}{r|}{\textbf{17.88}} &
  396.0 &
  \multicolumn{1}{r|}{18.55} &
  NA &
  NA \\
c-fat500-10 &
  500 &
  46627 &
  252 &
  19719 &
  \textbf{0.318} &
  \multicolumn{1}{r|}{1.961} &
  8.193 &
  \multicolumn{1}{r|}{\textbf{0.647}} &
  10.37 &
  1.471 &
  500 &
  46627 &
  \textbf{1783} &
  \multicolumn{1}{r|}{\textbf{332.9}} &
  1786 &
  \multicolumn{1}{r|}{373.9} &
  NA &
  NA \\
chesapeake &
  39 &
  170 &
  12 &
  43 &
  \textbf{0.026} &
  \multicolumn{1}{r|}{\textbf{0.001}} &
  0.177 &
  \multicolumn{1}{r|}{\textbf{0.001}} &
  0.803 &
  0.004 &
  26 &
  119 &
  \textbf{0.087} &
  \multicolumn{1}{r|}{\textbf{0.002}} &
  0.293 &
  \multicolumn{1}{r|}{0.004} &
  14556 &
  151.1 \\
delaunay\_n12 &
  4096 &
  12264 &
  4096 &
  12264 &
  \textbf{16.51} &
  \multicolumn{1}{r|}{\textbf{4.610}} &
  17.6 &
  \multicolumn{1}{r|}{16.13} &
  5567 &
  580.2 &
  4046 &
  12114 &
  \textbf{24.89} &
  \multicolumn{1}{r|}{\textbf{3.782}} &
  27.08 &
  \multicolumn{1}{r|}{16.57} &
  NA &
  NA \\
fe-sphere &
  16386 &
  49152 &
  16386 &
  49152 &
  \textbf{23.85} &
  \multicolumn{1}{r|}{\textbf{11.46}} &
  179.6 &
  \multicolumn{1}{r|}{909.8} &
  NA &
  NA &
  16386 &
  49152 &
  \textbf{331.6} &
  \multicolumn{1}{r|}{\textbf{62.56}} &
  332.6 &
  \multicolumn{1}{r|}{883.1} &
  NA &
  NA \\
hamming6-4 &
  64 &
  704 &
  64 &
  480 &
  \textbf{5.455} &
  \multicolumn{1}{r|}{0.041} &
  NA &
  \multicolumn{1}{r|}{NA} &
  4.569 &
  \textbf{0.024} &
  64 &
  480 &
  \textbf{68.40} &
  \multicolumn{1}{r|}{\textbf{0.667}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
rgg\_n\_2\_17\_s0 &
  131070 &
  728753 &
  135 &
  936 &
  \textbf{0.219} &
  \multicolumn{1}{r|}{\textbf{22.51}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  654 &
  4643 &
  \textbf{2.082} &
  \multicolumn{1}{r|}{\textbf{43.87}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-BU10 &
  19700 &
  637528 &
  5605 &
  121757 &
  \textbf{44.36} &
  \multicolumn{1}{r|}{\textbf{520.3}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  5414 &
  137711 &
  \textbf{105.2} &
  \multicolumn{1}{r|}{\textbf{553.9}} &
  397.9 &
  \multicolumn{1}{r|}{3555} &
  NA &
  NA \\
socfb-Cal65 &
  11247 &
  351358 &
  1288 &
  33884 &
  \textbf{9.192} &
  \multicolumn{1}{r|}{\textbf{101.2}} &
  101.3 &
  \multicolumn{1}{r|}{868.8} &
  NA &
  NA &
  1841 &
  50983 &
  \textbf{33.00} &
  \multicolumn{1}{r|}{\textbf{116.6}} &
  214.8 &
  \multicolumn{1}{r|}{782} &
  NA &
  NA \\
socfb-OR &
  63392 &
  816886 &
  5425 &
  132570 &
  \textbf{483.1} &
  \multicolumn{1}{r|}{\textbf{1663}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  3698 &
  98791 &
  \textbf{1439} &
  \multicolumn{1}{r|}{\textbf{1339}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-Penn94 &
  41536 &
  1362220 &
  6021 &
  162390 &
  \textbf{30.20} &
  \multicolumn{1}{r|}{\textbf{1528}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  4054 &
  117357 &
  \textbf{57.35} &
  \multicolumn{1}{r|}{\textbf{771.1}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-UCF52 &
  14940 &
  428989 &
  5241 &
  185956 &
  \textbf{80.27} &
  \multicolumn{1}{r|}{\textbf{770.0}} &
  421.4 &
  \multicolumn{1}{r|}{2050} &
  NA &
  NA &
  5195 &
  203128 &
  \textbf{296.5} &
  \multicolumn{1}{r|}{\textbf{1029}} &
  500.6 &
  \multicolumn{1}{r|}{2063} &
  NA &
  NA \\
socfb-UCSB37 &
  14917 &
  482215 &
  810 &
  27649 &
  \textbf{6.518} &
  \multicolumn{1}{r|}{\textbf{102.7}} &
  280.4 &
  \multicolumn{1}{r|}{2817} &
  NA &
  NA &
  627 &
  21724 &
  \textbf{5.193} &
  \multicolumn{1}{r|}{\textbf{58.89}} &
  292.8 &
  \multicolumn{1}{r|}{1955} &
  NA &
  NA \\
socfb-Vermont70 &
  7324 &
  191221 &
  4880 &
  122665 &
  \textbf{42.23} &
  \multicolumn{1}{r|}{\textbf{114.7}} &
  105.2 &
  \multicolumn{1}{r|}{268.3} &
  NA &
  NA &
  6036 &
  180323 &
  \textbf{103.0} &
  \multicolumn{1}{r|}{\textbf{154.2}} &
  120.6 &
  \multicolumn{1}{r|}{220.9} &
  NA &
  NA \\
socfb-wosn-friends &
  63731 &
  817090 &
  5425 &
  132570 &
  \textbf{483.1} &
  \multicolumn{1}{r|}{\textbf{1911}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  3698 &
  98791 &
  \textbf{1439} &
  \multicolumn{1}{r|}{\textbf{1914}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
web-BerkStan &
  12305 &
  19500 &
  8816 &
  16011 &
  \textbf{41.98} &
  \multicolumn{1}{r|}{\textbf{8.958}} &
  59.52 &
  \multicolumn{1}{r|}{370.3} &
  NA &
  NA &
  8816 &
  16011 &
  \textbf{109.2} &
  \multicolumn{1}{r|}{\textbf{26.98}} &
  167.9 &
  \multicolumn{1}{r|}{460.9} &
  NA &
  NA \\
web-indochina-2004 &
  11358 &
  47606 &
  203 &
  4117 &
  \textbf{0.220} &
  \multicolumn{1}{r|}{\textbf{2.708}} &
  81.49 &
  \multicolumn{1}{r|}{296.3} &
  7322 &
  1733 &
  452 &
  8129 &
  \textbf{1.171} &
  \multicolumn{1}{r|}{\textbf{4.006}} &
  183.7 &
  \multicolumn{1}{r|}{375.0} &
  NA &
  NA \\
web-webbase-2001 &
  16062 &
  25593 &
  1357 &
  5576 &
  \textbf{4.852} &
  \multicolumn{1}{r|}{\textbf{2.863}} &
  67.94 &
  \multicolumn{1}{r|}{766.1} &
  NA &
  NA &
  2793 &
  8953 &
  \textbf{36.63} &
  \multicolumn{1}{r|}{\textbf{4.685}} &
  237.4 &
  \multicolumn{1}{l|}{972.6} &
  NA &
  NA
\\\bottomrule
\end{tabular}
}
\vspace{-0.5em}\caption{Detailed results of MSB, RDS and \name on 25 representative MBP instances from four benchmarks for $s=2$ and $s=8$. The search tree size is in $10^3$, and the time is in seconds. The best results appear in bold.\vspace{-1em}}
\label{tab-comp-instances}
\end{table*}

==> tabs/compare-intances2.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[]
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l|rr|rrrrrrrr|rrrrrrrr}\toprule
\multirow{3}{*}{Instance} &
  \multicolumn{1}{r}{\multirow{3}{*}{$|V|$}} &
  \multicolumn{1}{r|}{\multirow{3}{*}{$|E|$}} &
  \multicolumn{8}{c|}{$s=2$} &
  \multicolumn{8}{c}{$s=8$} \\ \cline{4-19} 
 &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{4}{c|}{\name} &
  \multicolumn{2}{c|}{MSB} &
  \multicolumn{2}{c|}{RDS} &
  \multicolumn{4}{c|}{\name} &
  \multicolumn{2}{c|}{MSB} &
  \multicolumn{2}{c}{RDS} \\
 &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{r}{$|V'|$} &
  \multicolumn{1}{r}{$|E'|$} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r|}{Time} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r|}{Time} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r|}{Time} &
  \multicolumn{1}{r}{$|V'|$} &
  \multicolumn{1}{r}{$|E'|$} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r|}{Time} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r|}{Time} &
  \multicolumn{1}{r}{Tree} &
  \multicolumn{1}{r}{Time} \\ \hline
c-fat500-1 &
  500 &
  4459 &
  140 &
  1351 &
  \textbf{0.294} &
  \multicolumn{1}{r|}{\textbf{0.035}} &
  1.669 &
  \multicolumn{1}{r|}{0.117} &
  19.84 &
  0.301 &
  500 &
  4459 &
  \textbf{350.0} &
  \multicolumn{1}{r|}{\textbf{17.88}} &
  396.0 &
  \multicolumn{1}{r|}{18.55} &
  NA &
  NA \\
hamming6-4 &
  64 &
  704 &
  64 &
  480 &
  \textbf{5.455} &
  \multicolumn{1}{r|}{\textbf{0.041}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  4.569 &
  0.024 &
  64 &
  480 &
  \textbf{68.40} &
  \multicolumn{1}{r|}{\textbf{0.667}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
c-fat200-5 &
  200 &
  8473 &
  116 &
  4147 &
  \textbf{0.148} &
  \multicolumn{1}{r|}{\textbf{0.147}} &
  2.164 &
  \multicolumn{1}{r|}{0.049} &
  2.565 &
  0.083 &
  200 &
  8473 &
  \textbf{1720} &
  \multicolumn{1}{r|}{\textbf{75.78}} &
  1724 &
  \multicolumn{1}{r|}{81.74} &
  NA &
  NA \\
c-fat500-10 &
  500 &
  46627 &
  252 &
  19719 &
  \textbf{0.318} &
  \multicolumn{1}{r|}{1.961} &
  8.193 &
  \multicolumn{1}{r|}{\textbf{0.647}} &
  10.37 &
  1.471 &
  500 &
  46627 &
  \textbf{1783} &
  \multicolumn{1}{r|}{\textbf{332.9}} &
  1786 &
  \multicolumn{1}{r|}{373.9} &
  NA &
  NA \\
c-fat200-1 &
  200 &
  1534 &
  90 &
  729 &
  \textbf{0.001} &
  \multicolumn{1}{r|}{\textbf{0.011}} &
  0.704 &
  \multicolumn{1}{r|}{0.019} &
  3.757 &
  0.031 &
  200 &
  1534 &
  \textbf{28.63} &
  \multicolumn{1}{r|}{\textbf{0.954}} &
  32.23 &
  \multicolumn{1}{r|}{0.976} &
  NA &
  NA \\
bio-pdb1HYS &
  36417 &
  36417 &
  189 &
  4341 &
  \textbf{0.322} &
  \multicolumn{1}{r|}{\textbf{0.750}} &
  8.889 &
  \multicolumn{1}{r|}{2.936} &
  NA &
  NA &
  60 &
  1632 &
  \textbf{10.76} &
  \multicolumn{1}{r|}{\textbf{2.699}} &
  498.4 &
  \multicolumn{1}{r|}{28.65} &
  NA &
  NA \\
chesapeake &
  39 &
  170 &
  12 &
  43 &
  \textbf{0.026} &
  \multicolumn{1}{r|}{\textbf{0.001}} &
  0.177 &
  \multicolumn{1}{r|}{\textbf{0.001}} &
  0.803 &
 0.004 &
  26 &
  119 &
  \textbf{0.087} &
  \multicolumn{1}{r|}{\textbf{0.002}} &
  0.293 &
  \multicolumn{1}{r|}{0.004} &
  14556 &
  151.1 \\
delaunay\_n12 &
  4096 &
  12264 &
  4096 &
  12264 &
  \textbf{16.51} &
  \multicolumn{1}{r|}{\textbf{4.610}} &
  17.6 &
  \multicolumn{1}{r|}{16.13} &
  5567 &
  580.2 &
  4046 &
  12114 &
  \textbf{24.89} &
  \multicolumn{1}{r|}{\textbf{3.782}} &
  27.08 &
  \multicolumn{1}{r|}{16.57} &
  NA &
  NA \\
fe-sphere &
  16386 &
  49152 &
  16386 &
  49152 &
  \textbf{23.85} &
  \multicolumn{1}{r|}{\textbf{11.46}} &
  179.6 &
  \multicolumn{1}{r|}{909.8} &
  NA &
  NA &
  16386 &
  49152 &
  \textbf{331.6} &
  \multicolumn{1}{r|}{\textbf{62.56}} &
  332.6 &
  \multicolumn{1}{r|}{883.1} &
  NA &
  NA \\
rgg\_n\_2\_17\_s0 &
  131070 &
  728753 &
  135 &
  936 &
  \textbf{0.219} &
  \multicolumn{1}{r|}{\textbf{22.51}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  654 &
  4643 &
  \textbf{2.082} &
  \multicolumn{1}{r|}{\textbf{43.87}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
web-BerkStan &
  12305 &
  19500 &
  8816 &
  16011 &
  \textbf{41.98} &
  \multicolumn{1}{r|}{\textbf{8.958}} &
  59.52 &
  \multicolumn{1}{r|}{370.3} &
  NA &
  NA &
  8816 &
  16011 &
  \textbf{109.2} &
  \multicolumn{1}{r|}{\textbf{26.98}} &
  167.9 &
  \multicolumn{1}{r|}{460.9} &
  NA &
  NA \\
web-webbase-2001 &
  16062 &
  25593 &
  1357 &
  5576 &
  \textbf{4.852} &
  \multicolumn{1}{r|}{\textbf{2.863}} &
  67.94 &
  \multicolumn{1}{r|}{766.1} &
  NA &
  NA &
  2793 &
  8953 &
  \textbf{36.63} &
  \multicolumn{1}{r|}{\textbf{4.685}} &
  237.4 &
  \multicolumn{1}{l|}{972.6} &
  NA &
  NA \\
web-indochina-2004 &
  11358 &
  47606 &
  203 &
  4117 &
  \textbf{0.220} &
  \multicolumn{1}{r|}{\textbf{2.708}} &
  81.49 &
  \multicolumn{1}{r|}{296.3} &
  7322 &
  1733 &
  452 &
  8129 &
  \textbf{1.171} &
  \multicolumn{1}{r|}{\textbf{4.006}} &
  183.7 &
  \multicolumn{1}{r|}{375.0} &
  NA &
  NA \\
bio-dmela &
  7393 &
  25569 &
  151 &
  621 &
  \textbf{0.522} &
  \multicolumn{1}{r|}{\textbf{0.217}} &
  149.8 &
  \multicolumn{1}{r|}{94.61} &
  8983 &
  1494 &
  2288 &
  15498 &
  \textbf{1695} &
  \multicolumn{1}{r|}{\textbf{119.5}} &
  1807 &
  \multicolumn{1}{r|}{338.5} &
  NA &
  NA \\
ca-AstroPh &
  17903 &
  196972 &
  113 &
  3136 &
  \textbf{0.060} &
  \multicolumn{1}{r|}{\textbf{4.070}} &
  91.52 &
  \multicolumn{1}{r|}{1377} &
  NA &
  NA &
  267 &
  7269 &
  \textbf{1.093} &
  \multicolumn{1}{r|}{\textbf{8.628}} &
  476.9 &
  \multicolumn{1}{r|}{1862} &
  NA &
  NA \\
socfb-BU10 &
  19700 &
  637528 &
  5605 &
  121757 &
  \textbf{44.36} &
  \multicolumn{1}{r|}{\textbf{520.3}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  5414 &
  137711 &
  \textbf{105.2} &
  \multicolumn{1}{r|}{\textbf{553.9}} &
  397.9 &
  \multicolumn{1}{r|}{3555} &
  NA &
  NA \\
socfb-Cal65 &
  11247 &
  351358 &
  1288 &
  33884 &
  \textbf{9.192} &
  \multicolumn{1}{r|}{\textbf{101.2}} &
  101.3 &
  \multicolumn{1}{r|}{868.8} &
  NA &
  NA &
  1841 &
  50983 &
  \textbf{33.00} &
  \multicolumn{1}{r|}{\textbf{116.6}} &
  214.8 &
  \multicolumn{1}{r|}{782.0} &
  NA &
  NA \\
socfb-UCF52 &
  14940 &
  428989 &
  5241 &
  185956 &
  \textbf{80.27} &
  \multicolumn{1}{r|}{\textbf{770.0}} &
  421.4 &
  \multicolumn{1}{r|}{2050} &
  NA &
  NA &
  5195 &
  203128 &
  \textbf{296.5} &
  \multicolumn{1}{r|}{\textbf{1029}} &
  500.6 &
  \multicolumn{1}{r|}{2063} &
  NA &
  NA \\
socfb-UCSB37 &
  14917 &
  482215 &
  810 &
  27649 &
  \textbf{6.518} &
  \multicolumn{1}{r|}{\textbf{102.7}} &
  280.4 &
  \multicolumn{1}{r|}{2817} &
  NA &
  NA &
  627 &
  21724 &
  \textbf{5.193} &
  \multicolumn{1}{r|}{\textbf{58.89}} &
  292.8 &
  \multicolumn{1}{r|}{1955} &
  NA &
  NA \\
socfb-Vermont70 &
  7324 &
  191221 &
  4880 &
  122665 &
  \textbf{42.23} &
  \multicolumn{1}{r|}{\textbf{114.7}} &
  105.2 &
  \multicolumn{1}{r|}{268.3} &
  NA &
  NA &
  6036 &
  180323 &
  \textbf{103.0} &
  \multicolumn{1}{r|}{\textbf{154.2}} &
  120.6 &
  \multicolumn{1}{r|}{220.9} &
  NA &
  NA \\
ca-dblp-2010 &
  226413 &
  716460 &
  455 &
  13491 &
  \textbf{0.574} &
  \multicolumn{1}{r|}{\textbf{272.9}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  844 &
  21716 &
  \textbf{2.327} &
  \multicolumn{1}{r|}{\textbf{327.6}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
ca-dblp-2012 &
  317080 &
  1049866 &
  216 &
  11592 &
  \textbf{0.106} &
  \multicolumn{1}{r|}{\textbf{448.6}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  216 &
  11592 &
  \textbf{0.160} &
  \multicolumn{1}{r|}{\textbf{396.0}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-OR &
  63392 &
  816886 &
  5425 &
  132570 &
  \textbf{483.1} &
  \multicolumn{1}{r|}{\textbf{1663}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  3698 &
  98791 &
  \textbf{1439} &
  \multicolumn{1}{r|}{\textbf{1339}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-Penn94 &
  41536 &
  1362220 &
  6021 &
  162390 &
  \textbf{30.20} &
  \multicolumn{1}{r|}{\textbf{1528}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  4054 &
  117357 &
  \textbf{57.35} &
  \multicolumn{1}{r|}{\textbf{771.1}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA \\
socfb-wosn-friends &
  63731 &
  817090 &
  5425 &
  132570 &
  \textbf{483.1} &
  \multicolumn{1}{r|}{\textbf{1911}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA &
  3698 &
  98791 &
  \textbf{1439} &
  \multicolumn{1}{r|}{\textbf{1914}} &
  NA &
  \multicolumn{1}{r|}{NA} &
  NA &
  NA
\\\bottomrule
\end{tabular}
}
\caption{Detailed results of MSB, RDS and \name on 25 representative MBP instances from four benchmarks with $s=2$ and $s=8$. The search tree size is in $10^3$, and the time is in seconds. The best results appear in bold.}
\label{tab-comp-instances}
\end{table*}
